Barium stars as tracers of s-process nucleosynthesis in AGB stars II. Using machine learning techniques on 169 stars

We aim to analyse the abundance pattern of 169 Barium (Ba) stars, using machine learning techniques and the AGB final surface abundances predicted by Fruity and Monash stellar models. We developed machine learning algorithms that use the abundance pattern of Ba stars as input to classify the initial mass and metallicity of its companion star using stellar model predictions. We use two algorithms: the first exploits neural networks to recognise patterns and the second is a nearest-neighbour algorithm, which focuses on finding the AGB model that predicts final surface abundances closest to the observed Ba star values. In the second algorithm we include the error bars and observational uncertainties to find the best fit model. The classification process is based on the abundances of Fe, Rb, Sr, Zr, Ru, Nd, Ce, Sm, and Eu. We selected these elements by systematically removing s-process elements from our AGB model abundance distributions, and identifying those whose removal has the biggest positive effect on the classification. We excluded Nb, Y, Mo, and La. Our final classification combines the output of both algorithms to identify for each Ba star companion an initial mass and metallicity range. With our analysis tools we identify the main properties for 166 of the 169 Ba stars in the stellar sample. The classifications based on both stellar sets of AGB final abundances show similar distributions, with an average initial mass of M = 2.23 MSun and 2.34 MSun and an average [Fe/H] = -0.21 and -0.11, respectively. We investigated why the removal of Nb, Y, Mo, and La improves our classification and identified 43 stars for which the exclusion had the biggest effect. We show that these stars have statistically significant different abundances for these elements compared to the other Ba stars in our sample. We discuss the possible reasons for these differences in the abundance patterns.

==> Latex_table_28matchedstars_F.tex <==
\begin{longtable}{l|llll}
\caption{This table lists the subset of 28 Ba stars and their FRUITY classifications.}\label{tab:fruity28}\\ 
Star & Mass range (Mo) & Metallicity range (Z) & minimum GoF & agreement Cseh+2021\\ 
\hline
BD $-$14$^{\circ}$2678 & 2.25--2.75 & 0.0059--0.017 & 84.58 & $-$0.37 -0.3\\\ 
CD $-$42$^{\circ}$2048 & 2.25 - 2.75 & 0.0059 - 0.017 & 63.9 & n\\ 
CPD $-$64$^{\circ}$4333 & 2.25 - 2.75 & 0.0035 - 0.0102 & 64.32 & y\\ 
HD 20394 & 2.25--2.75 & 0.0035 - 0.0136 & 72 & n\\ 
HD 24035 & 1.25 - 2.75 & 0.0035 - 0.0136 & 55 & y\\ 
HD 40430 & 2.25 - 2.75 & 0.0059 - 0.017 & 93 & y\\ 
HD 49641 & 2.75 - 4.25 & 0.0035 - 0.0102 & 83 & y\\
HD 58368 & 2.25 - 3.25 & 0.0059 - 0.017 & 64 & -\\ 
HD 59852 & 2.25 - 2.75 & 0.0059 - 0.017 & 94 & y\\ 
HD 84678 & 1.75 - 2.25 & 0.0035 - 0.0102 & 50 & -\\ 
HD 91208 & 1.75 - 2.75 & 0.0059 - 0.017 & 71 & -\\ 
HD 92626 & 2.25 - 2.75 & 0.0035 - 0.0102 & 57 & y\\ 
HD 107541 & 2.25 - 2.75 & 0.0035 - 0.0102 & 62 & -\\ 
HD 119185 & 2.25 - 2.75 & 0.0059 - 0.0102 & 65 & n\\ 
HD 143899 & 1.75 - 2.25 & 0.0047 - 0.017 & 88 & n\\ 
HD 154430 & 1.25 - 1.75 & 0.0047 - 0.0136 & 96 & -\\ 
HD 183915 & 1.25 - 2.25 & 0.0035 - 0.0102 & 89 & y\\ 
HD 201657 & 1.75 - 2.75 & 0.0047 - 0.0136 & 97 & y\\ 
HD 201824 & 1.75 - 2.25 & 0.0047 - 0.0136 & 96 & n\\ 
HD 210946 & 2.25 - 2.75 & 0.0059 - 0.017 & 83 & n\\ 
HD 211594 & 2.25 - 2.75 & 0.0047 - 0.0136 & 87 & -\\ 
HD 18182 & 2.25 - 2.75 & 0.0082 - 0.0238 & 78 & -\\ 
HD 53199 & 2.25 - 2.75 & 0.0059 - 0.017 & 85 & y\\ 
HD 58121 & 1.75 - 2.25 & 0.0082 - 0.017 & 79 & y\\ 
HD 95193 & 2.25 - 2.75 & 0.0082 - 0.017 & 94 & n\\ 
HD 134698 & 1.25 - 1.55 & 0.0047 - 0.0102 & 82 & -\\ 
HD 180622 & 1.75 - 2.25 & 0.0082 - 0.017 & 92 & y\\ 
HD 200063 & 1.75 - 2.25 & 0.0059 - 0.0136 & 98 & y\\ 
\end{longtable}

==> Latex_table_28matchedstars_M.tex <==
\begin{longtable}{l|llll}
\caption{This table lists the subset of 28 Ba stars and their matched MONASH models.}\label{tab:monash28}\\ 
Star & Mass range (M$_{\odot}$) & Metallicity range ([Fe/H]) & minimum GoF & agreement Cseh+2021\\ 
\hline
BD $-$14$^{\circ}$2678 & 1.75 - 2.25 & 0.0082 - 0.0238 & 97.54 & n\\ 
CD $-$42$^{\circ}$2048 & 1.75 - 2.5 & 0.0082 - 0.0238 & 55.95 & n\\ 
CPD $-$64$^{\circ}$4333 & 1.75 - 3.0 & 0.0041 - 0.0238 & 76.8 & y\\ 
HD 20394 & 1.75 - 2.25 & 0.0059 - 0.017 & 82 & n\\ 
HD 24035 & 1.65 - 2.5 & 0.0041 - 0.0119 & 80 & y\\ 
HD 40430 & 1.75 - 2.25 & 0.0082 - 0.017 & 88 & n\\  
HD 49641 & 4.25 - 4.75 & 0.0041 - 0.0119 & 89 & n\\ 
HD 58368 & - & - & - & -\\ 
HD 59852 & 2.25 - 3.25 & 0.0082 - 0.017 & 91 & y\\ 
HD 84678 & 1.5 - 2.5 & 0.0082 - 0.0119 & 52 & -\\ 
HD 91208 & 1.75 - 2.5 & 0.0082 - 0.0238 & 84 & -\\ 
HD 92626 & 1.75 - 2.5 & 0.0041 - 0.0119 & 95 & -\\ 
HD 107541 & 2.25 - 2.75 & 0.0041 - 0.0048 & 88 & -\\ 
HD 119185 & 1.75 - 2.25 & 0.0082 - 0.0119 & 62 & n\\ 
HD 143899 & 1.75 - 2.25 & 0.0082 - 0.017 & 86 & n\\ 
HD 154430 & 1.5 - 2.25 & 0.0059 - 0.0119 & 95 & -\\ 
HD 183915 & 1.25 - 2.35 & 0.0041 - 0.0119 & 91 & y\\ 
HD 201657 & 1.75 - 3.0 & 0.0041 - 0.017 & 96 & y\\ 
HD 201824 & 1.75 - 2.25 & 0.0059 - 0.0119 & 97 & y\\ 
HD 210946 & 1.75 - 3.25 & 0.0082 - 0.0238 & 82 & y\\ 
HD 211594 & 2.5 - 3.0 & 0.0041 - 0.0119 & 83 & y\\ 
HD 18182 & 2.5 - 2.75 & 0.0176 - 0.0238 & 68 & -\\ 
HD 53199 & 1.75 - 2.25 & 0.0082 - 0.017 & 74 & n\\ 
HD 58121 & 1.75 - 2.75 & 0.0082 - 0.0238 & 80 & y\\ 
HD 95193 & 1.75 - 2.5 & 0.0082 - 0.0238 & 98 & n\\ 
HD 134698 & 3.25 - 3.75 & 0.0082 - 0.0119 & 83 & -\\ 
HD 180622 & 1.75 - 3.0 & 0.0082 - 0.0238 & 91 & - \\ 
HD 200063 & 1.75 - 2.25 & 0.0082 - 0.0119 & 96 & y\\ 
\end{longtable}

==> Latex_table_missing_matchedstars_F.tex <==
%\begin{longtable}{l|llll}
\begin{table*}
\centering
\caption{This table lists the stars and their matched FRUITY models.}
\begin{tabular}{l|llll}
Star & Mass range (M$_{\odot}$) & Metallicity range ([Fe/H]) & minimum GoF & missing elements\\ 
\hline
HD 4084 & - & - & - & -\\ 
HD 49641 & 2.75 to 4.25 & -0.6 to -0.14 & 83 & Rb\\
HD 66291 & - & - & - & -\\ 
HD 123396 & - & - & - & -\\ 
HD 177192 & - & - & - & Eu \\ 
HD 204075 & 2.25 to 2.75 & -0.23 to 0.23 & 97 & Ru\\ 
HD 219116 & - & - & - & -\\
MFU 112 & - & - & - & -\\
HD 21682 & 2.25 to 2.75 & -0.6 to -0.14 & 76 & Ru\\ 
HD 49661 & 1.25 to 2.25 & -0.38 to -0.01 & 72 & Eu \\ 
HD 62017 & - & - & - & -\\
HD107270 & - & - & - & -\\
HD 148892 & - & - & - & Rb\\ 
BD +09$^{\circ}$2384 & - & - & - & Sr, Ru\\ 
%\end{longtable}
\end{tabular}

\label{tab:missing_fruity}
\end{table*}

==> Latex_table_missing_matchedstars_M.tex <==
%\begin{longtable}{l|llll}
\begin{table*}
\centering
\caption{This table lists the stars and their matched MONASH models.}
\begin{tabular}{l|llll}
Star & Mass range (M$_{\odot}$) & Metallicity range ([Fe/H]) & minimum GoF & missing elements\\ 
\hline
HD 49641 & 4.25 to 4.75 & -0.54 to -0.07 & 89 & Rb\\
HD 58368 & - & - & - & -\\ 
HD 123396 & - & - & - & -\\ 
HD 130255 & - & - & - & -\\ 
HD 177192 & 2.5 to 2.75 & -0.23 to 0.23 & 74 & Eu  \\ 
HD 204075 & 2.5 to 2.75 & 0.1 to 0.23 & 98 & Ru\\ 
HD 219116 & - & - & - & -\\ 
HD 21682 & 1.75 to 2.5 & -0.54 to -0.07 & 78 & Ru\\ 
HD 33709 & - & - & - & -\\ 
HD 49661 & 1.75 to 2.5 & -0.23 to 0.23 & 67 & Eu \\ 
HD 62017 & - & - & - & -\\ 
HD 148892 & 4.75 to 4.75 & -0.54 to -0.07 & 71 & Rb\\ 
BD +09$^{\circ}$2384 & - & - & - & Sr, Ru\\ 
%\end{longtable}
\end{tabular}

\label{tab:missing_monash}
\end{table*}

==> corr_mat_all.tex <==
\begin{landscape}\begin{longtable}{l|ccccccccccccccccccccc}
\caption{This is the covariance matrix of all the elements.}\label{tab:names}\\ 
&Fe/H&Rb/Fe&Sr/Fe&Nb/Fe&Mo/Fe&Ru/Fe&La/Fe&Sm/Fe&Eu/Fe&Na&Mg&Al&Si&Ca&Ti&Cr&Ni&Y&Zr&Ce&Nd \\ 
\hline
Fe/H & 1.0 & -0.3 & -0.3 & -0.4 & -0.2 & -0.2 & -0.3 & -0.3 & -0.5 & -0.1 & -0.8 & -0.4 & -0.6 & 0.0 & -0.6 & -0.2 & -0.3 & -0.2 & -0.3 & -0.4 & -0.4\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Rb/Fe & -0.3 & 1.0 & 0.5 & 0.5 & 0.5 & 0.4 & 0.5 & 0.5 & 0.5 & 0.0 & 0.1 & 0.1 & 0.3 & -0.0 & 0.4 & 0.1 & 0.2 & 0.6 & 0.5 & 0.5 & 0.6\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Sr/Fe & -0.3 & 0.5 & 1.0 & 0.7 & 0.8 & 0.7 & 0.9 & 0.8 & 0.8 & 0.0 & 0.3 & 0.3 & 0.3 & -0.0 & 0.5 & 0.3 & 0.0 & 0.8 & 0.9 & 0.9 & 0.9\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Nb/Fe & -0.4 & 0.5 & 0.7 & 1.0 & 0.8 & 0.8 & 0.9 & 0.9 & 0.9 & -0.0 & 0.2 & 0.3 & 0.2 & 0.0 & 0.5 & 0.2 & -0.0 & 0.8 & 0.9 & 0.9 & 0.9\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Mo/Fe & -0.2 & 0.5 & 0.8 & 0.8 & 1.0 & 0.8 & 0.9 & 0.9 & 0.8 & -0.1 & 0.1 & 0.3 & 0.3 & 0.0 & 0.5 & 0.2 & 0.0 & 0.9 & 0.9 & 0.8 & 0.8\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Ru/Fe & -0.2 & 0.4 & 0.7 & 0.8 & 0.8 & 1.0 & 0.8 & 0.8 & 0.8 & -0.2 & 0.2 & 0.1 & 0.1 & -0.0 & 0.4 & 0.1 & 0.1 & 0.7 & 0.8 & 0.7 & 0.7\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
La/Fe & -0.3 & 0.5 & 0.9 & 0.9 & 0.9 & 0.8 & 1.0 & 0.9 & 0.9 & -0.1 & 0.2 & 0.4 & 0.2 & -0.1 & 0.4 & 0.2 & 0.0 & 0.9 & 1.0 & 1.0 & 1.0\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Sm/Fe & -0.3 & 0.5 & 0.8 & 0.9 & 0.9 & 0.8 & 0.9 & 1.0 & 0.9 & 0.0 & 0.2 & 0.4 & 0.3 & -0.0 & 0.4 & 0.3 & 0.0 & 0.8 & 0.9 & 0.9 & 0.9\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Eu/Fe & -0.5 & 0.5 & 0.8 & 0.9 & 0.8 & 0.8 & 0.9 & 0.9 & 1.0 & -0.1 & 0.3 & 0.4 & 0.3 & -0.1 & 0.5 & 0.1 & 0.2 & 0.8 & 0.9 & 0.9 & 0.9\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Na & -0.1 & 0.0 & 0.0 & -0.0 & -0.1 & -0.2 & -0.1 & 0.0 & -0.1 & 1.0 & 0.1 & 0.2 & 0.5 & 0.7 & 0.2 & 0.3 & 0.1 & -0.2 & -0.0 & -0.1 & -0.0\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Mg & -0.8 & 0.1 & 0.3 & 0.2 & 0.1 & 0.2 & 0.2 & 0.2 & 0.3 & 0.1 & 1.0 & 0.4 & 0.4 & -0.0 & 0.4 & 0.3 & 0.2 & 0.1 & 0.2 & 0.3 & 0.2\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Al & -0.4 & 0.1 & 0.3 & 0.3 & 0.3 & 0.1 & 0.4 & 0.4 & 0.4 & 0.2 & 0.4 & 1.0 & 0.3 & 0.2 & 0.3 & 0.2 & 0.1 & 0.3 & 0.3 & 0.4 & 0.4\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Si & -0.6 & 0.3 & 0.3 & 0.2 & 0.3 & 0.1 & 0.2 & 0.3 & 0.3 & 0.5 & 0.4 & 0.3 & 1.0 & 0.4 & 0.8 & 0.2 & 0.6 & 0.2 & 0.3 & 0.3 & 0.3\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Ca & 0.0 & -0.0 & -0.0 & 0.0 & 0.0 & -0.0 & -0.1 & -0.0 & -0.1 & 0.7 & -0.0 & 0.2 & 0.4 & 1.0 & 0.3 & -0.2 & 0.4 & -0.0 & -0.0 & -0.1 & -0.1\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Ti & -0.6 & 0.4 & 0.5 & 0.5 & 0.5 & 0.4 & 0.4 & 0.4 & 0.5 & 0.2 & 0.4 & 0.3 & 0.8 & 0.3 & 1.0 & 0.2 & 0.6 & 0.5 & 0.5 & 0.4 & 0.4\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Cr & -0.2 & 0.1 & 0.3 & 0.2 & 0.2 & 0.1 & 0.2 & 0.3 & 0.1 & 0.3 & 0.3 & 0.2 & 0.2 & -0.2 & 0.2 & 1.0 & -0.3 & 0.2 & 0.3 & 0.3 & 0.3\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Ni & -0.3 & 0.2 & 0.0 & -0.0 & 0.0 & 0.1 & 0.0 & 0.0 & 0.2 & 0.1 & 0.2 & 0.1 & 0.6 & 0.4 & 0.6 & -0.3 & 1.0 & -0.0 & 0.0 & 0.0 & -0.0\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Y & -0.2 & 0.6 & 0.8 & 0.8 & 0.9 & 0.7 & 0.9 & 0.8 & 0.8 & -0.2 & 0.1 & 0.3 & 0.2 & -0.0 & 0.5 & 0.2 & -0.0 & 1.0 & 0.9 & 0.8 & 0.8\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Zr & -0.3 & 0.5 & 0.9 & 0.9 & 0.9 & 0.8 & 1.0 & 0.9 & 0.9 & -0.0 & 0.2 & 0.3 & 0.3 & -0.0 & 0.5 & 0.3 & 0.0 & 0.9 & 1.0 & 0.9 & 0.9\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Ce & -0.4 & 0.5 & 0.9 & 0.9 & 0.8 & 0.7 & 1.0 & 0.9 & 0.9 & -0.1 & 0.3 & 0.4 & 0.3 & -0.1 & 0.4 & 0.3 & 0.0 & 0.8 & 0.9 & 1.0 & 1.0\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
Nd & -0.4 & 0.6 & 0.9 & 0.9 & 0.8 & 0.7 & 1.0 & 0.9 & 0.9 & -0.0 & 0.2 & 0.4 & 0.3 & -0.1 & 0.4 & 0.3 & -0.0 & 0.8 & 0.9 & 1.0 & 1.0\\ 
&&&&&&&&&&&&&&&&&&&&&\\ 
\end{longtable}\end{landscape}

==> names.tex <==
\begin{longtable}{ll} 
\caption{This table lists the full and short names of the AGB models.} \label{tab:names}\\ 
 Short name &Full name \\ 
\hline
F-m1.3z0003a & fruity\_m1p3z3m4\_000\\ 
F-m1.3z001a & fruity\_m1p3z1m3\_000\\ 
F-m1.3z002a & fruity\_m1p3z2m3\_000\\ 
F-m1.3z003a & fruity\_m1p3z3m3\_000\\ 
F-m1.3z006a & fruity\_m1p3z6m3\_000\\ 
F-m1.3z008a & fruity\_m1p3z8m3\_000\\ 
F-m1.5z0003a & fruity\_m1p5z3m4\_T60\\ 
F-m1.5z0003b & fruity\_m1p5z3m4\_060\\ 
F-m1.5z0003c & fruity\_m1p5z3m4\_000\\ 
F-m1.5z001a & fruity\_m1p5z1m3\_ext\\ 
F-m1.5z001b & fruity\_m1p5z1m3\_060\\ 
F-m1.5z001c & fruity\_m1p5z1m3\_T60\\ 
F-m1.5z001d & fruity\_m1p5z1m3\_000\\ 
F-m1.5z002a & fruity\_m1p5z2m3\_000\\ 
F-m1.5z002b & fruity\_m1p5z2m3\_ext\\ 
F-m1.5z003a & fruity\_m1p5z3m3\_060\\ 
F-m1.5z003b & fruity\_m1p5z3m3\_000\\ 
F-m1.5z003c & fruity\_m1p5z3m3\_ext\\ 
F-m1.5z006a & fruity\_m1p5z6m3\_ext\\ 
F-m1.5z006b & fruity\_m1p5z6m3\_000\\ 
F-m1.5z006c & fruity\_m1p5z6m3\_060\\ 
F-m1.5z008a & fruity\_m1p5z8m3\_000\\ 
F-m1.5z014a & fruity\_m1p5zsun\_000\\ 
F-m1.5z01a & fruity\_m1p5z1m2\_ext\\ 
F-m1.5z01b & fruity\_m1p5z1m2\_060\\ 
F-m1.5z01c & fruity\_m1p5z1m2\_T60\\ 
F-m1.5z01d & fruity\_m1p5z1m2\_000\\ 
F-m1.5z02a & fruity\_m1p5z2m2\_000\\ 
F-m2.0z0003a & fruity\_m2p0z3m4\_000\\ 
F-m2.0z001a & fruity\_m2p0z1m3\_ext\\ 
F-m2.0z001b & fruity\_m2p0z1m3\_000\\ 
F-m2.0z002a & fruity\_m2p0z2m3\_000\\ 
F-m2.0z003a & fruity\_m2p0z3m3\_000\\ 
F-m2.0z003b & fruity\_m2p0z3m3\_ext\\ 
F-m2.0z006a & fruity\_m2p0z6m3\_ext\\ 
F-m2.0z006b & fruity\_m2p0z6m3\_000\\ 
F-m2.0z008a & fruity\_m2p0z8m3\_000\\ 
F-m2.0z014a & fruity\_m2p0zsun\_060\\ 
F-m2.0z014b & fruity\_m2p0zsun\_000\\ 
F-m2.0z014c & fruity\_m2p0zsun\_010\\ 
F-m2.0z014d & fruity\_m2p0zsun\_030\\ 
F-m2.0z014e & fruity\_m2p0zsun\_ext\\ 
F-m2.0z01a & fruity\_m2p0z1m2\_ext\\ 
F-m2.0z01b & fruity\_m2p0z1m2\_T60\\ 
F-m2.0z01c & fruity\_m2p0z1m2\_000\\ 
F-m2.0z02a & fruity\_m2p0z2m2\_000\\ 
F-m2.5z0003a & fruity\_m2p5z3m4\_000\\ 
F-m2.5z001a & fruity\_m2p5z1m3\_000\\ 
F-m2.5z002a & fruity\_m2p5z2m3\_000\\ 
F-m2.5z003a & fruity\_m2p5z3m3\_000\\ 
F-m2.5z006a & fruity\_m2p5z6m3\_000\\ 
F-m2.5z008a & fruity\_m2p5z8m3\_000\\ 
F-m2.5z014a & fruity\_m2p5zsun\_000\\ 
F-m2.5z01a & fruity\_m2p5z1m2\_000\\ 
F-m2.5z02a & fruity\_m2p5z2m2\_000\\ 
F-m3.0z0003a & fruity\_m3p0z3m4\_000\\ 
F-m3.0z001a & fruity\_m3p0z1m3\_000\\ 
F-m3.0z002a & fruity\_m3p0z2m3\_000\\ 
F-m3.0z003a & fruity\_m3p0z3m3\_000\\ 
F-m3.0z006a & fruity\_m3p0z6m3\_000\\ 
F-m3.0z008a & fruity\_m3p0z8m3\_000\\ 
F-m3.0z014a & fruity\_m3p0zsun\_000\\ 
F-m3.0z01a & fruity\_m3p0z1m2\_000\\ 
F-m3.0z02a & fruity\_m3p0z2m2\_000\\ 
F-m4.0z0003a & fruity\_m4p0z3m4\_000\\ 
F-m4.0z001a & fruity\_m4p0z1m3\_000\\ 
F-m4.0z002a & fruity\_m4p0z2m3\_000\\ 
F-m4.0z003a & fruity\_m4p0z3m3\_000\\ 
F-m4.0z006a & fruity\_m4p0z6m3\_000\\ 
F-m4.0z008a & fruity\_m4p0z8m3\_000\\ 
F-m4.0z014a & fruity\_m4p0zsun\_000\\ 
F-m4.0z01a & fruity\_m4p0z1m2\_000\\ 
F-m4.0z02a & fruity\_m4p0z2m2\_000\\ 
F-m5.0z0003a & fruity\_m5p0z3m4\_000\\ 
F-m5.0z001a & fruity\_m5p0z1m3\_000\\ 
F-m5.0z002a & fruity\_m5p0z2m3\_000\\ 
F-m5.0z003a & fruity\_m5p0z3m3\_000\\ 
F-m5.0z006a & fruity\_m5p0z6m3\_000\\ 
F-m5.0z008a & fruity\_m5p0z8m3\_000\\ 
F-m5.0z014a & fruity\_m5p0zsun\_000\\ 
F-m5.0z01a & fruity\_m5p0z1m2\_000\\ 
F-m6.0z0003a & fruity\_m6p0z3m4\_000\\ 
F-m6.0z001a & fruity\_m6p0z1m3\_000\\ 
F-m6.0z002a & fruity\_m6p0z2m3\_000\\ 
F-m6.0z006a & fruity\_m6p0z6m3\_000\\ 
F-m6.0z008a & fruity\_m6p0z8m3\_000\\ 
F-m6.0z01a & fruity\_m6p0z1m2\_000\\ 
\hline \hline
M-m1.25z0028a & monash\_m1.25\_mix\_2.00E-03\_z0028\\ 
M-m1.25z0028b & monash\_m1.25\_mix\_6.00E-03\_z0028\\ 
M-m1.5z0028a & monash\_m1.50\_mix\_2.00E-03\_z0028\\ 
M-m1.5z0028b & monash\_m1.50\_mix\_6.00E-03\_z0028\\ 
M-m1.5z007a & monash\_m1.50\_mix\_2.00E-03\_N\_ov\_0.0\_z007\\ 
M-m1.5z007b & monash\_m1.50\_mix\_2.00E-03\_N\_ov\_1.0\_z007\\ 
M-m1.5z014a & monash\_m1.50\_mix\_2.00E-03\_N\_ov\_3.0\_z014\\ 
M-m1.75z0028a & monash\_m1.75\_mix\_2.00E-03\_z0028\\ 
M-m1.75z007a & monash\_m1.75\_mix\_2.00E-03\_N\_ov\_0.0\_z007\\ 
M-m1.75z007b & monash\_m1.75\_mix\_2.00E-03\_N\_ov\_1.0\_z007\\ 
M-m1.75z014a & monash\_m1.75\_mix\_2.00E-03\_N\_ov\_2.0\_z014\\ 
M-m1.9z007a & monash\_m1.90\_mix\_2.00E-03\_z007\\ 
M-m2.0z0028a & monash\_m2.00\_mix\_2.00E-03\_z0028\\ 
M-m2.0z0028b & monash\_m2.00\_mix\_6.00E-03\_z0028\\ 
M-m2.0z014a & monash\_m2.00\_mix\_1.00E-03\_z014\\ 
M-m2.0z014b & monash\_m2.00\_mix\_2.00E-03\_z014\\ 
M-m2.0z014c & monash\_m2.00\_mix\_4.00E-03\_z014\\ 
M-m2.0z01a & monash\_m2.00\_mix\_2.00E-03\_z01\\ 
M-m2.1z007a & monash\_m2.10\_mix\_2.00E-03\_z007\\ 
M-m2.25z0028a & monash\_m2.25\_mix\_2.00E-03\_z0028\\ 
M-m2.25z007a & monash\_m2.25\_mix\_2.00E-03\_z007\\ 
M-m2.25z014a & monash\_m2.25\_mix\_2.00E-03\_z014\\ 
M-m2.5z0028a & monash\_m2.50\_mix\_2.00E-03\_z0028\\ 
M-m2.5z0028b & monash\_m2.50\_mix\_4.00E-03\_z0028\\ 
M-m2.5z007a & monash\_m2.50\_mix\_2.00E-03\_z007\\ 
M-m2.5z014a & monash\_m2.50\_mix\_2.00E-03\_z014\\ 
M-m2.5z03a & monash\_m2.50\_mix\_2.00E-03\_N\_ov\_2.5\_z03\\ 
M-m2.75z0028a & monash\_m2.75\_mix\_2.00E-03\_z0028\\ 
M-m2.75z007a & monash\_m2.75\_mix\_2.00E-03\_z007\\ 
M-m2.75z014a & monash\_m2.75\_mix\_2.00E-03\_z014\\ 
M-m2.75z03a & monash\_m2.75\_mix\_2.00E-03\_N\_ov\_0.0\_z03\\ 
M-m2.75z03b & monash\_m2.75\_mix\_2.00E-03\_N\_ov\_2.0\_z03\\ 
M-m3.0z0028a & monash\_m3.00\_mix\_1.00E-03\_z0028\\ 
M-m3.0z0028b & monash\_m3.00\_mix\_2.00E-03\_z0028\\ 
M-m3.0z007a & monash\_m3.00\_mix\_1.00E-03\_z007\\ 
M-m3.0z007b & monash\_m3.00\_mix\_2.00E-03\_z007\\ 
M-m3.0z014a & monash\_m3.00\_mix\_1.00E-04\_z014\\ 
M-m3.0z014b & monash\_m3.00\_mix\_1.00E-03\_z014\\ 
M-m3.0z014c & monash\_m3.00\_mix\_2.00E-03\_z014\\ 
M-m3.0z01a & monash\_m3.00\_mix\_2.00E-03\_z01\\ 
M-m3.0z03a & monash\_m3.00\_mix\_2.00E-03\_N\_ov\_0.0\_z03\\ 
M-m3.0z03b & monash\_m3.00\_mix\_2.00E-03\_N\_ov\_1.0\_z03\\ 
M-m3.25z0028a & monash\_m3.25\_mix\_1.00E-03\_z0028\\ 
M-m3.25z007a & monash\_m3.25\_mix\_1.00E-03\_z007\\ 
M-m3.25z014a & monash\_m3.25\_mix\_1.00E-03\_z014\\ 
M-m3.25z014b & monash\_m3.25\_mix\_2.00E-03\_z014\\ 
M-m3.25z03a & monash\_m3.25\_mix\_1.00E-03\_z03\\ 
M-m3.25z03b & monash\_m3.25\_mix\_2.00E-03\_z03\\ 
M-m3.5z0028a & monash\_m3.50\_mix\_1.00E-03\_z0028\\ 
M-m3.5z007a & monash\_m3.50\_mix\_1.00E-03\_z007\\ 
M-m3.5z014a & monash\_m3.50\_mix\_1.00E-03\_z014\\ 
M-m3.5z03a & monash\_m3.50\_mix\_1.00E-03\_z03\\ 
M-m3.75z007a & monash\_m3.75\_mix\_1.00E-03\_z007\\ 
M-m3.75z014a & monash\_m3.75\_mix\_1.00E-03\_z014\\ 
M-m3.75z03a & monash\_m3.75\_mix\_1.00E-03\_z03\\ 
M-m4.0z0028a & monash\_m4.00\_mix\_1.00E-04\_z0028\\ 
M-m4.0z007a & monash\_m4.00\_mix\_1.00E-04\_z007\\ 
M-m4.0z007b & monash\_m4.00\_mix\_1.00E-03\_z007\\ 
M-m4.0z014a & monash\_m4.00\_mix\_1.00E-04\_z014\\ 
M-m4.0z014b & monash\_m4.00\_mix\_1.00E-03\_z014\\ 
M-m4.0z03a & monash\_m4.00\_mix\_1.00E-03\_z03\\ 
M-m4.25z007a & monash\_m4.25\_mix\_1.00E-04\_z007\\ 
M-m4.25z014a & monash\_m4.25\_mix\_1.00E-04\_z014\\ 
M-m4.25z014b & monash\_m4.25\_mix\_1.00E-03\_z014\\ 
M-m4.25z03a & monash\_m4.25\_mix\_1.00E-04\_z03\\ 
M-m4.25z03b & monash\_m4.25\_mix\_1.00E-03\_z03\\ 
M-m4.5z0028a & monash\_m4.50\_mix\_0.00E+00\_z0028\\ 
M-m4.5z0028b & monash\_m4.50\_mix\_1.00E-04\_z0028\\ 
M-m4.5z007a & monash\_m4.50\_mix\_0.00E+00\_z007\\ 
M-m4.5z007b & monash\_m4.50\_mix\_1.00E-04\_z007\\ 
M-m4.5z014a & monash\_m4.50\_mix\_1.00E-04\_z014\\ 
M-m4.5z014b & monash\_m4.50\_mix\_1.00E-03\_z014\\ 
M-m4.5z03a & monash\_m4.50\_mix\_1.00E-04\_z03\\ 
M-m4.5z03b & monash\_m4.50\_mix\_1.00E-03\_z03\\ 
M-m4.75z007a & monash\_m4.75\_mix\_0.00E+00\_z007\\ 
M-m4.75z014a & monash\_m4.75\_mix\_1.00E-04\_z014\\ 
M-m4.75z03a & monash\_m4.75\_mix\_1.00E-04\_z03\\ 
M-m5.0z0028a & monash\_m5.00\_mix\_0.00E+00\_z0028\\ 
M-m5.0z007a & monash\_m5.00\_mix\_0.00E+00\_z007\\ 
M-m5.0z014a & monash\_m5.00\_mix\_1.00E-04\_z014\\ 
M-m5.0z03a & monash\_m5.00\_mix\_1.00E-04\_z03\\ 
M-m5.5z0028a & monash\_m5.50\_mix\_0.00E+00\_z0028\\ 
M-m5.5z007a & monash\_m5.50\_mix\_0.00E+00\_z007\\ 
M-m5.5z014a & monash\_m5.50\_mix\_0.00E+00\_z014\\ 
M-m6.0z0028a & monash\_m6.00\_mix\_0.00E+00\_z0028\\ 
M-m6.0z007a & monash\_m6.00\_mix\_0.00E+00\_z007\\ 
M-m6.5z0028a & monash\_m6.50\_mix\_0.00E+00\_z0028\\ 
M-m7.0z0028a & monash\_m7.00\_mix\_0.00E+00\_z0028\\ 
M-m7.0z007a & monash\_m7.00\_mix\_0.00E+00\_z007\\ 
M-m7.0z014a & monash\_m7.00\_mix\_0.00E+00\_z014\\ 
M-m7.5z007a & monash\_m7.50\_mix\_0.00E+00\_z007\\ 
M-m8.0z014a & monash\_m8.00\_mix\_0.00E+00\_z014\\ 
M-m8.0z03a & monash\_m8.00\_mix\_0.00E+00\_z03\\ 
\hline
\end{longtable}

==> names_table.tex <==
\begin{longtable}{ll}[B]
\centering
\caption{This table lists the full and short names of the AGB models.}\label{tab:names}\\ 
 Short name & Full name \\ 
\hline
F-m1.3z0003a & fruity\_m1p3z3m4\_000\\ 
F-m1.3z001a & fruity\_m1p3z1m3\_000\\ 
F-m1.3z002a & fruity\_m1p3z2m3\_000\\ 
F-m1.3z003a & fruity\_m1p3z3m3\_000\\ 
F-m1.3z006a & fruity\_m1p3z6m3\_000\\ 
F-m1.3z008a & fruity\_m1p3z8m3\_000\\ 
F-m1.5z0003a & fruity\_m1p5z3m4\_T60\\ 
F-m1.5z0003b & fruity\_m1p5z3m4\_060\\ 
F-m1.5z0003c & fruity\_m1p5z3m4\_000\\ 
F-m1.5z001a & fruity\_m1p5z1m3\_ext\\
F-m1.5z001b & fruity\_m1p5z1m3\_060\\ 
F-m1.5z001c & fruity\_m1p5z1m3\_T60\\ 
F-m1.5z001d & fruity\_m1p5z1m3\_000\\ 
F-m1.5z002a & fruity\_m1p5z2m3\_000\\ 
F-m1.5z002b & fruity\_m1p5z2m3\_ext\\ 
F-m1.5z003a & fruity\_m1p5z3m3\_060\\ 
F-m1.5z003b & fruity\_m1p5z3m3\_000\\ 
F-m1.5z003c & fruity\_m1p5z3m3\_ext\\ 
F-m1.5z006a & fruity\_m1p5z6m3\_ext\\ 
F-m1.5z006b & fruity\_m1p5z6m3\_000\\ 
F-m1.5z006c & fruity\_m1p5z6m3\_060\\ 
F-m1.5z008a & fruity\_m1p5z8m3\_000\\ 
F-m1.5z014a & fruity\_m1p5zsun\_000\\ 
F-m1.5z01a & fruity\_m1p5z1m2\_ext\\ 
F-m1.5z01b & fruity\_m1p5z1m2\_060\\ 
F-m1.5z01c & fruity\_m1p5z1m2\_T60\\ 
F-m1.5z01d & fruity\_m1p5z1m2\_000\\ 
F-m1.5z02a & fruity\_m1p5z2m2\_000\\ 
F-m2.0z0003a & fruity\_m2p0z3m4\_000\\ 
F-m2.0z001a & fruity\_m2p0z1m3\_ext\\ 
F-m2.0z001b & fruity\_m2p0z1m3\_000\\ 
F-m2.0z002a & fruity\_m2p0z2m3\_000\\ 
F-m2.0z003a & fruity\_m2p0z3m3\_000\\ 
F-m2.0z003b & fruity\_m2p0z3m3\_ext\\ 
F-m2.0z006a & fruity\_m2p0z6m3\_ext\\ 
F-m2.0z006b & fruity\_m2p0z6m3\_000\\ 
F-m2.0z008a & fruity\_m2p0z8m3\_000\\ 
F-m2.0z014a & fruity\_m2p0zsun\_060\\ 
F-m2.0z014b & fruity\_m2p0zsun\_000\\ 
F-m2.0z014c & fruity\_m2p0zsun\_010\\ 
F-m2.0z014d & fruity\_m2p0zsun\_030\\ 
F-m2.0z014e & fruity\_m2p0zsun\_ext\\ 
F-m2.0z01a & fruity\_m2p0z1m2\_ext\\ 
F-m2.0z01b & fruity\_m2p0z1m2\_T60\\ 
F-m2.0z01c & fruity\_m2p0z1m2\_000\\ 
F-m2.0z02a & fruity\_m2p0z2m2\_000\\ 
F-m2.5z0003a & fruity\_m2p5z3m4\_000\\ 
F-m2.5z001a & fruity\_m2p5z1m3\_000\\ 
F-m2.5z002a & fruity\_m2p5z2m3\_000\\ 
F-m2.5z003a & fruity\_m2p5z3m3\_000\\ 
F-m2.5z006a & fruity\_m2p5z6m3\_000\\ 
F-m2.5z008a & fruity\_m2p5z8m3\_000\\ 
F-m2.5z014a & fruity\_m2p5zsun\_000\\ 
F-m2.5z01a & fruity\_m2p5z1m2\_000\\ 
F-m2.5z02a & fruity\_m2p5z2m2\_000\\ 
F-m3.0z0003a & fruity\_m3p0z3m4\_000\\ 
F-m3.0z001a & fruity\_m3p0z1m3\_000\\ 
F-m3.0z002a & fruity\_m3p0z2m3\_000\\ 
F-m3.0z003a & fruity\_m3p0z3m3\_000\\ 
F-m3.0z006a & fruity\_m3p0z6m3\_000\\ 
F-m3.0z008a & fruity\_m3p0z8m3\_000\\ 
F-m3.0z014a & fruity\_m3p0zsun\_000\\ 
F-m3.0z01a & fruity\_m3p0z1m2\_000\\ 
F-m3.0z02a & fruity\_m3p0z2m2\_000\\ 
F-m4.0z0003a & fruity\_m4p0z3m4\_000\\ 
F-m4.0z001a & fruity\_m4p0z1m3\_000\\ 
F-m4.0z002a & fruity\_m4p0z2m3\_000\\ 
F-m4.0z003a & fruity\_m4p0z3m3\_000\\ 
F-m4.0z006a & fruity\_m4p0z6m3\_000\\ 
F-m4.0z008a & fruity\_m4p0z8m3\_000\\ 
F-m4.0z014a & fruity\_m4p0zsun\_000\\ 
F-m4.0z01a & fruity\_m4p0z1m2\_000\\ 
F-m4.0z02a & fruity\_m4p0z2m2\_000\\ 
F-m5.0z0003a & fruity\_m5p0z3m4\_000\\ 
F-m5.0z001a & fruity\_m5p0z1m3\_000\\ 
F-m5.0z002a & fruity\_m5p0z2m3\_000\\ 
F-m5.0z003a & fruity\_m5p0z3m3\_000\\ 
F-m5.0z006a & fruity\_m5p0z6m3\_000\\ 
F-m5.0z008a & fruity\_m5p0z8m3\_000\\ 
F-m5.0z014a & fruity\_m5p0zsun\_000\\ 
F-m5.0z01a & fruity\_m5p0z1m2\_000\\ 
F-m6.0z0003a & fruity\_m6p0z3m4\_000\\ 
F-m6.0z001a & fruity\_m6p0z1m3\_000\\ 
F-m6.0z002a & fruity\_m6p0z2m3\_000\\ 
F-m6.0z006a & fruity\_m6p0z6m3\_000\\ 
F-m6.0z008a & fruity\_m6p0z8m3\_000\\ 
F-m6.0z01a & fruity\_m6p0z1m2\_000\\ 
M-m1.25z0028a & monash\_m1.25\_mix\_2.00E-03\_z0028\\ 
M-m1.25z0028b & monash\_m1.25\_mix\_6.00E-03\_z0028\\ 
M-m1.50z0028a & monash\_m1.50\_mix\_2.00E-03\_z0028\\ 
M-m1.50z0028b & monash\_m1.50\_mix\_6.00E-03\_z0028\\ 
M-m1.50z007a & monash\_m1.50\_mix\_2.00E-03\_N\_ov\_0.0\_z007\\ 
M-m1.50z007b & monash\_m1.50\_mix\_2.00E-03\_N\_ov\_1.0\_z007\\ 
M-m1.50z014a & monash\_m1.50\_mix\_2.00E-03\_N\_ov\_3.0\_z014\\ 
M-m1.75z0028a & monash\_m1.75\_mix\_2.00E-03\_z0028\\ 
M-m1.75z007a & monash\_m1.75\_mix\_2.00E-03\_N\_ov\_0.0\_z007\\ 
M-m1.75z007b & monash\_m1.75\_mix\_2.00E-03\_N\_ov\_1.0\_z007\\ 
M-m1.75z014a & monash\_m1.75\_mix\_2.00E-03\_N\_ov\_2.0\_z014\\ 
M-m1.90z007a & monash\_m1.90\_mix\_2.00E-03\_z007\\ 
M-m2.00z0028a & monash\_m2.00\_mix\_2.00E-03\_z0028\\ 
M-m2.00z0028b & monash\_m2.00\_mix\_6.00E-03\_z0028\\ 
M-m2.00z014a & monash\_m2.00\_mix\_1.00E-03\_z014\\ 
M-m2.00z014b & monash\_m2.00\_mix\_2.00E-03\_z014\\ 
M-m2.00z014c & monash\_m2.00\_mix\_4.00E-03\_z014\\ 
M-m2.00z01a & monash\_m2.00\_mix\_2.00E-03\_z01\\ 
M-m2.10z007a & monash\_m2.10\_mix\_2.00E-03\_z007\\ 
M-m2.25z0028a & monash\_m2.25\_mix\_2.00E-03\_z0028\\ 
M-m2.25z007a & monash\_m2.25\_mix\_2.00E-03\_z007\\ 
M-m2.25z014a & monash\_m2.25\_mix\_2.00E-03\_z014\\ 
M-m2.50z0028a & monash\_m2.50\_mix\_2.00E-03\_z0028\\ 
M-m2.50z0028b & monash\_m2.50\_mix\_4.00E-03\_z0028\\ 
M-m2.50z007a & monash\_m2.50\_mix\_2.00E-03\_z007\\ 
M-m2.50z014a & monash\_m2.50\_mix\_2.00E-03\_z014\\ 
M-m2.50z03a & monash\_m2.50\_mix\_2.00E-03\_N\_ov\_2.5\_z03\\ 
M-m2.75z0028a & monash\_m2.75\_mix\_2.00E-03\_z0028\\ 
M-m2.75z007a & monash\_m2.75\_mix\_2.00E-03\_z007\\ 
M-m2.75z014a & monash\_m2.75\_mix\_2.00E-03\_z014\\ 
M-m2.75z03a & monash\_m2.75\_mix\_2.00E-03\_N\_ov\_0.0\_z03\\ 
M-m2.75z03b & monash\_m2.75\_mix\_2.00E-03\_N\_ov\_2.0\_z03\\ 
M-m3.00z0028a & monash\_m3.00\_mix\_1.00E-03\_z0028\\ 
M-m3.00z0028b & monash\_m3.00\_mix\_2.00E-03\_z0028\\ 
M-m3.00z007a & monash\_m3.00\_mix\_1.00E-03\_z007\\ 
M-m3.00z007b & monash\_m3.00\_mix\_2.00E-03\_z007\\ 
M-m3.00z014a & monash\_m3.00\_mix\_1.00E-04\_z014\\ 
M-m3.00z014b & monash\_m3.00\_mix\_1.00E-03\_z014\\ 
M-m3.00z014c & monash\_m3.00\_mix\_2.00E-03\_z014\\ 
M-m3.00z01a & monash\_m3.00\_mix\_2.00E-03\_z01\\ 
M-m3.00z03a & monash\_m3.00\_mix\_2.00E-03\_N\_ov\_0.0\_z03\\ 
M-m3.00z03b & monash\_m3.00\_mix\_2.00E-03\_N\_ov\_1.0\_z03\\ 
M-m3.25z0028a & monash\_m3.25\_mix\_1.00E-03\_z0028\\ 
M-m3.25z007a & monash\_m3.25\_mix\_1.00E-03\_z007\\ 
M-m3.25z014a & monash\_m3.25\_mix\_1.00E-03\_z014\\ 
M-m3.25z014b & monash\_m3.25\_mix\_2.00E-03\_z014\\ 
M-m3.25z03a & monash\_m3.25\_mix\_1.00E-03\_z03\\ 
M-m3.25z03b & monash\_m3.25\_mix\_2.00E-03\_z03\\ 
M-m3.50z0028a & monash\_m3.50\_mix\_1.00E-03\_z0028\\ 
M-m3.50z007a & monash\_m3.50\_mix\_1.00E-03\_z007\\ 
M-m3.50z014a & monash\_m3.50\_mix\_1.00E-03\_z014\\ 
M-m3.50z03a & monash\_m3.50\_mix\_1.00E-03\_z03\\ 
M-m3.75z007a & monash\_m3.75\_mix\_1.00E-03\_z007\\ 
M-m3.75z014a & monash\_m3.75\_mix\_1.00E-03\_z014\\ 
M-m3.75z03a & monash\_m3.75\_mix\_1.00E-03\_z03\\ 
M-m4.00z0028a & monash\_m4.00\_mix\_1.00E-04\_z0028\\ 
M-m4.00z007a & monash\_m4.00\_mix\_1.00E-04\_z007\\ 
M-m4.00z007b & monash\_m4.00\_mix\_1.00E-03\_z007\\ 
M-m4.00z014a & monash\_m4.00\_mix\_1.00E-04\_z014\\ 
M-m4.00z014b & monash\_m4.00\_mix\_1.00E-03\_z014\\ 
M-m4.00z03a & monash\_m4.00\_mix\_1.00E-03\_z03\\ 
M-m4.25z007a & monash\_m4.25\_mix\_1.00E-04\_z007\\ 
M-m4.25z014a & monash\_m4.25\_mix\_1.00E-04\_z014\\ 
M-m4.25z014b & monash\_m4.25\_mix\_1.00E-03\_z014\\ 
M-m4.25z03a & monash\_m4.25\_mix\_1.00E-04\_z03\\ 
M-m4.25z03b & monash\_m4.25\_mix\_1.00E-03\_z03\\ 
M-m4.50z0028a & monash\_m4.50\_mix\_0.00E+00\_z0028\\ 
M-m4.50z0028b & monash\_m4.50\_mix\_1.00E-04\_z0028\\ 
M-m4.50z007a & monash\_m4.50\_mix\_0.00E+00\_z007\\ 
M-m4.50z007b & monash\_m4.50\_mix\_1.00E-04\_z007\\ 
M-m4.50z014a & monash\_m4.50\_mix\_1.00E-04\_z014\\ 
M-m4.50z014b & monash\_m4.50\_mix\_1.00E-03\_z014\\ 
M-m4.50z03a & monash\_m4.50\_mix\_1.00E-04\_z03\\ 
M-m4.50z03b & monash\_m4.50\_mix\_1.00E-03\_z03\\ 
M-m4.75z007a & monash\_m4.75\_mix\_0.00E+00\_z007\\ 
M-m4.75z014a & monash\_m4.75\_mix\_1.00E-04\_z014\\ 
M-m4.75z03a & monash\_m4.75\_mix\_1.00E-04\_z03\\ 
M-m5.00z0028a & monash\_m5.00\_mix\_0.00E+00\_z0028\\ 
M-m5.00z007a & monash\_m5.00\_mix\_0.00E+00\_z007\\ 
M-m5.00z014a & monash\_m5.00\_mix\_1.00E-04\_z014\\ 
M-m5.00z03a & monash\_m5.00\_mix\_1.00E-04\_z03\\ 
M-m5.50z0028a & monash\_m5.50\_mix\_0.00E+00\_z0028\\ 
M-m5.50z007a & monash\_m5.50\_mix\_0.00E+00\_z007\\ 
M-m5.50z014a & monash\_m5.50\_mix\_0.00E+00\_z014\\ 
M-m6.00z0028a & monash\_m6.00\_mix\_0.00E+00\_z0028\\ 
M-m6.00z007a & monash\_m6.00\_mix\_0.00E+00\_z007\\ 
M-m6.50z0028a & monash\_m6.50\_mix\_0.00E+00\_z0028\\ 
M-m7.00z0028a & monash\_m7.00\_mix\_0.00E+00\_z0028\\ 
M-m7.00z007a & monash\_m7.00\_mix\_0.00E+00\_z007\\ 
M-m7.00z014a & monash\_m7.00\_mix\_0.00E+00\_z014\\ 
M-m7.50z007a & monash\_m7.50\_mix\_0.00E+00\_z007\\ 
M-m8.00z014a & monash\_m8.00\_mix\_0.00E+00\_z014\\ 
M-m8.00z03a & monash\_m8.00\_mix\_0.00E+00\_z03\\ 
\hline
\end{longtable}
